Superconductivity in the Correlated Pyrochlore Cd_2Re_2O_7

We report the observation of superconductivity in high-quality Cd$_2$Re$_2$O$_7$ single crystals with room-temperature pyrochlore structure. Resistivity and ac susceptibility measurements establish an onset transition temperature T$_c^{onset}$ = 1.47 K with transition width $\Delta$T$_c$ = 0.25 K. In applied magnetic field, the resistive transition shows a type-II character, with an approximately linear temperature-dependence of the upper critical field H$_{c2}$. The bulk nature of the superconductivity is confirmed by the specific heat jump with $\Delta$C = 37.9 mJ/mol-K. Using the $\gamma$ value extracted from normal-state specific heat data, we obtain $\Delta$C/$\gamma$T$_c$ = 1.29, close to the weak coupling BCS value. In the normal state, a negative Hall coefficient below 100 K suggests electron-like conduction in this material. The resistivity exhibits a quadratic T-dependence between 2 and 60 K, i.e., $\rho =\rho_0$+AT$^2$, indicative of Fermi-liquid behavior. The values of the Kadowaki-Woods ratio A/$\gamma^2$ and the Wilson ratio are comparable to that for strongly correlated materials.

==> Cd2Re2O7bib.tex <==
@ARTICLE{mandrus,
   author = "D. Mandrus and J.R. Thompson and R. Gaal and L. Forro and C.J. Bryan and B.C. Chakoumakos and L.M. Woods and B.C. Sales and R.S. Fishman and V. Keppens",
   year = "2001",
   journal = "Phys. Rev. B",
   volume = "63",
   pages = "195104"
}

 @ARTICLE{subr,
    author = "{For a review, see M.A. Subramanian and G. Aravamudan and G.V. Subba
Rao}",
    year = "1983",
    journal = "Prog. Solid State Chem.",
   volume = "15",
   pages = "55"
}

 @ARTICLE{donohue,
   author = "P.C. Donohue and J.M. Longo and R.D. Rosenstein and L. Katz",
   year = "1965",
   journal = "Inorg. Chem.",
   volume = "4",
   pages = "1152"
}

@ARTICLE{he,
   author = "{J. He {\it et al.}}",
   year = "2001",
  journal = "(to be submitted)" }

@ARTICLE{jin1,
    author = "{R. Jin {\it et al.}}",
    year = "2001",
    journal = "Bulletin of APS-March Meeting"
   volume = "46",
   pages = "1061"
}

@ARTICLE{jin2,
   author = "{R. Jin {\it et al.}}",
   year = "2001",
   journal = "(to be submitted)"
}

@ARTICLE{sakai,
   author = "{H. Sakai {\it et al.}}",
   year = "2001",
   journal = "cond-mat/0106521"
}

@ARTICLE{maeka,
   author = "S. Maekawa and H. Ebisawa and H. Fukuyama",
   year = "1983",
   journal = "J. Phys. Soc. Jpn.",
   volume = "52",
   pages = "1352"
}

 @ARTICLE{black,
   author = "{K. Blacklock and H.W. White}",
   year = "1979",
   journal = "J. Chem. Phys.",
   volume = "71",
   pages = "5287"
}
 @ARTICLE{ikeda,
   author = "S. Ikeda and Y. Maeno and H. Muranishi and T. Fujita",
   year = "1996",
   journal = "J. of Low Temp. Phys.",
   volume = "105",
   pages = "1599"
}

@ARTICLE{ikeda2,
   author = "{S. Ikeda and Y. Maeno and S. Nakatsuji and M. Kosaka and Y. Uwatoko}",
   year = "2000",
   journal = "Phys. Rev. B",
   volume = "62",
   pages = "6089"
}

 , ibid. 99, 457 (1996).

@ARTICLE{kw,
   author = "{K. Kadowaki and S.B. Woods}",
   year = "1986",
   journal = "Solid State Commun.",
   volume = "58",
   pages = "507"
}

@ARTICLE{miyaka,
   author = "{K. Miyaka and T. Matsuura and C.M. Varma}",
   year = "1989",
   journal = "Solid State Commun.",
   volume = "71",
   pages = "1149"
}

@ARTICLE{takimoto,
   author = "T. Takimoto and T. Moriya",
   year = "1996",
   journal = "Solid State Commun.",
   volume = "99",
   pages = "457"
}

@ARTICLE{whh,
   author = "N.R. Werthamer and E. Helfand and P.C. Hohenberg",
   year = "1966",
   journal = "Phys. Rev.",
   volume = "147",
   pages = "295"
}

@ARTICLE{kondo,
   author = "S. Kondo and D.C. Johnston and C.A. Swenson {\it et al.} ",
   year = "1997",
   journal = "Phys. Rev. Lett.",
   volume = "78",
   pages = "3729"
}

@ARTICLE{mackenzie,
   author = "A.P. Mackenzie and R.K.W. Haselwimmer and A.W. Tyler and G.G. Lonzarich and Y. Mori and S. Nishizaki and Y. Maeno ",
   year = "1998",
   journal = "Phys. Rev. Lett.",
   volume = "80",
   pages = "161"

}

@BOOK{anderson,
    author = "P.W. Anderson",
    title = "Theory of Superconductivity in High-T$_c$ Cuprates",
    publisher = "Princeton University Press",
    year = "1997",
    address = "Princeton"
}

@BOOK{tinkham,
    author = "M. Tinkham",
    title = "Introduction to Superconductivity",
    publisher = "McGraw-Hill",
    year = "1975",
    address = "New York"
}

@ARTICLE{ishii,
   author = "F. Ishii and T. Oguchi",
   year = "2000",
   journal = "J. Phys. Soc. Jpn.",
   volume = "69",
   pages = "526"

}

